LARGO: Low-Rank Hypernetwork for Handling Missing Modalities

Addressing missing modalities is an important challenge in multimodal image analysis and often relies on complex architectures that do not transfer easily to different datasets without architectural modifications or hyperparameter tuning. While most existing methods tackle this problem in feature space by engineering representations that are robust to missing inputs, we instead operate in weight space. We propose LARGO, a hypernetwork that compresses the $2^N-1$ dedicated missing-modality models into a single network by modelling the convolutional weights using the Canonical Polyadic (CP) tensor decomposition. Extensive experimental validation on BraTS 2018 (4 modalities, 15 scenarios) and ISLES 2022 (3 modalities, 7 scenarios) shows that our method ranks first in 47 out of 52 configurations, achieving average Dice improvements of +0.68$\%$ and +2.53$\%$ over state-of-the-art baselines (mmFormer, M$^{3}$AE, ShaSpec, SimMLM). A proof-of-concept experiment on avMNIST suggests that LARGO may extend beyond medical imaging to heterogeneous non-medical modalities. Code is available at https://github.com/nielsvyncke/LARGO.

==> Fig/methodology/palette.tex <==
% Shared palette and node styles of Figure 1 (camera-ready revision):
% amber = modalities / model selection, green = convolution kernels, purple = low-rank factors and
% hypernetwork layers, coral = stem, blue = head and output.
\definecolor{Amber}{RGB}{245,188,54}
\definecolor{AmberLight}{RGB}{255,226,150}
\definecolor{Missing}{RGB}{225,225,225}
\definecolor{Coral}{RGB}{250,150,140}
\definecolor{Leaf}{RGB}{160,220,160}
\definecolor{LeafDark}{RGB}{50,150,60}
\definecolor{Sky}{RGB}{140,190,240}
\definecolor{Violet}{RGB}{205,180,238}
\definecolor{VioletLight}{RGB}{238,230,250}
\definecolor{VioletDark}{RGB}{140,90,200}
\definecolor{Output}{RGB}{70,110,230}
\tikzset{
    >=stealth,
    box/.style={rounded corners=4pt, draw=black!30, fill=black!4},
    layer/.style={rounded corners=2pt, draw=black!45, thin},
    mod/.style={rounded corners=1pt, draw=black!45, thin},
    arr/.style={->, thick, black!60},
    brace/.style={decorate, decoration={brace, amplitude=5pt, mirror, raise=4pt}, thick, black!60},
    side/.style={rotate=90, font=\bfseries, text=black!75},
    bottom/.style={font=\bfseries, text=black!80},
    dots/.style={rotate=90, font=\bfseries, text=black!60},
    panel/.style={rounded corners=6pt, fill=black!3, draw=black!15},
    num/.style={circle, fill=black!75, text=white, inner sep=0pt, minimum size=0.42cm, font=\bfseries\footnotesize},
    ptitle/.style={anchor=west, font=\bfseries\small},
    fac/.style={circle, draw=black!55, thick, minimum size=0.72cm, inner sep=0pt},
    Afac/.style={fac, fill=AmberLight},
    Bfac/.style={fac, fill=Violet},
    Wfac/.style={fac, fill=Leaf},
    leg/.style={draw=black!65, thick},
    lab/.style={font=\footnotesize, inner sep=1.5pt},
    kern/.style={draw=black!50, thick, rounded corners=1pt},
    flow/.style={->, thick, black!65, shorten >=1pt},
    big/.style={-stealth, line width=1.6pt, black!40},
    note/.style={font=\scriptsize, text=black!70, align=center, inner sep=1pt},
    bus/.style={very thick, rounded corners}
}

